Streaming and Massively Parallel Algorithms for Euclidean Max-Cut

Given a set of vectors $X = \{ x_1,\dots, x_n \} \subset \mathbb{R}^d$, the Euclidean max-cut problem asks to partition the vectors into two parts so as to maximize the sum of Euclidean distances which cross the partition. We design new algorithms for Euclidean max-cut in models for massive datasets: $\bullet$ We give a fully-scalable constant-round MPC algorithm using $O(nd) + n \cdot \text{poly}( \log(n) / \epsilon)$ total space which gives a $(1+\epsilon)$-approximate Euclidean max-cut. $\bullet$ We give a dynamic streaming algorithm using $\text{poly}(d \log \Delta / \epsilon)$ space when $X \subseteq [\Delta]^d$, which provides oracle access to a $(1+\epsilon)$-approximate Euclidean max-cut. Recently, Chen, Jiang, and Krauthgamer $[\text{STOC}~'23]$ gave a dynamic streaming algorithm with space $\text{poly}(d\log\Delta/\epsilon)$ to approximate the value of the Euclidean max-cut, but could not provide oracle access to an approximately optimal cut. This was left open in that work, and we resolve it here. Both algorithms follow from the same framework, which analyzes a ``parallel'' and ``subsampled'' (Euclidean) version of a greedy algorithm of Mathieu and Schudy $[\text{SODA}~'08]$ for dense max-cut.

==> wrapping-seeded.tex <==
% !TEX root = main.tex

\section{Fully Scalable MPC Algorithm}

\begin{itemize}
\item Round 1: Compute a sketch to determine weights which are $\lambda$-compatible, and communicate the sketch.
\item Round 2: 
\begin{itemize}
\item Every point computes its own row of $\bA$ and $\bK$ (since they know the weights). They determine whether or not the point was sampled, and if a point was sampled, the information needed to communicate that sampled point is communicated to everyone.
\item In addition, if $m$ is the number of non-zero rows in the first $t_0$ columns of $\bA \circ \bK$, we take $O(m/\eps^2)$ geometric samples and communicate these as well.  
\end{itemize}
\end{itemize}
After this, each point may decide independently which side of the cut they belong to. First, they use the $O(m/\eps^2)$ geometric samples in order to agree on a setting of the seed $(\sigma, P)$, and then they each assign themselves to either side of the cut. 
